Consensus Time in 3-Majority and 2-Choices Is Determined by the Maximum Initial Opinion Density

We establish the correct parameter governing the convergence time of the 3-Majority and 2-Choices dynamics on the complete graph in the synchronous model. Recent work [Shimizu and Shiraga, PODC'25] provides matching upper and lower bounds on the number of rounds to consensus, but only in a weak sense: the bounds are shown to coincide for some initial opinion configuration. In contrast, we obtain tight bounds in a strong sense, with upper and lower bounds matching up to logarithmic factors for every initial configuration. Let $\alpha^{(0)}$ be the initial opinion-frequency vector, and denote by $\|\alpha^{(0)}\|_\infty$ its maximum entry. We show that 3-Majority reaches consensus in $\tilde{\Theta}(\min\{\|\alpha^{(0)}\|_\infty^{-1},\sqrt n\})$ rounds w.h.p., while 2-Choices reaches consensus in $\tilde{\Theta}(\|\alpha^{(0)}\|_\infty^{-1})$ rounds w.h.p. Our results demonstrate that the convergence time of both dynamics is governed not by global parameters such as the number of opinions $k$ or the squared $\ell_2$ norm of the initial opinion distribution, but rather by the ``local'' parameter $\|\alpha^{(0)}\|_\infty$, the maximum initial opinion density.

==> commands.tex <==
\RequirePackage{mathtools}
\RequirePackage{xspace}

\def\defeq{\mathrel{\mathop:}=}

%\DeclarePairedDelimiter{\abs}{\lvert}{\rvert} % | | absolute value
%\DeclarePairedDelimiter{\norm}{\lVert}{\rVert} % || || norm
\DeclarePairedDelimiter{\rbra}{\lparen}{\rparen} % () round brackets
\DeclarePairedDelimiter{\cbra}{\lbrace}{\rbrace} % {} curly brackets
\DeclarePairedDelimiter{\sbra}{\lbrack}{\rbrack} % [] square brackets
\DeclarePairedDelimiter{\abra}{\langle}{\rangle} % < > angle brackets
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor} % floor function
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil} % ceil function
\newcommand{\pa}[1]{\left(#1\right)}

\newcommand{\indicator}{\mathbf{1}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\opinions}{\mathcal{C}}
\newcommand{\alphavec}{\boldsymbol{\alpha}}
\newcommand{\whp}{with high probability}
\newcommand{\condition}{\;\middle\vert\;}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\e}{\mathrm{e}}
\renewcommand{\d}{\mathrm{d}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Int}{\mathbb{Z}}
\newcommand{\Comp}{\mathbb{C}}
\newcommand{\binset}{\{0,1 \}}
\newcommand{\intset}[1]{\{0, \ldots,  #1\}}
\newcommand{\numset}[1]{\{1, \ldots,  #1\}}
\DeclareMathOperator\polylog{polylog}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\KL}[2]{\mathrm{KL} \big(#1 \parallel #2\big) }

\newcommand{\Otilde}{\widetilde{O}}

\newcommand{\constref}[1]{C_{\mbox{\tiny\ref{#1}}}}
\newcommand{\constrefs}[2]{C_{\mbox{\tiny\ref{#1}(\ref{#2})}}}
\newcommand{\varianceref}[1]{\variance_{\mbox{\tiny\ref{#1}}}}
\newcommand{\driftref}[1]{\drift_{\mbox{\tiny\ref{#1}}}}
\newcommand{\Tref}[1]{T_{\mbox{\tiny\ref{#1}}}}

\newcommand{\calF}{\mathcal{F}}

\newcommand{\taucons}{\tau_{\mathrm{cons}}}
\newcommand{\alphanorm}{\gamma}

\newcommand{\taualphaup}{\tau^{\uparrow}_\alpha}
\newcommand{\taualphadown}{\tau^{\downarrow}_\alpha}
\newcommand{\taudeltaplus}{\tau^{+}_\delta}
\newcommand{\tauetaplus}{\tau^{+}_\eta}


\newcommand{\cweak}{c^{\mathrm{weak}}}
\newcommand{\calphaup}{c^{\uparrow}_\alpha}
\newcommand{\calphadown}{c^{\downarrow}_\alpha}
\newcommand{\cdeltaplus}{c^{+}_\delta}

\newcommand{\aratio}{R}
\newcommand{\opinion}{\mathsf{opn}}
\newcommand{\bounded}{D}
\newcommand{\variance}{s}
\newcommand{\constlemma}[1]{C_{\mbox{\tiny\ref{#1}}}}

\newcommand{\Bern}{\mathsf{Bern}}
\newcommand{\oneBern}{\mathsf{Bern}^+}

\newcommand{\taunormup}{\tau^{\uparrow}_\alphanorm}
\newcommand{\taunormdown}{\tau^{\downarrow}_\alphanorm}
\newcommand{\taunormplus}{\tau^{+}_{\alphanorm}}
\newcommand{\taudisappeari}{\tau^*_i}
\newcommand{\tauincreasei}{\tau^{\mathrm{active}}_i}
\newcommand{\calE}{\mathcal{E}}

\newcommand{\cnormup}{c^{\uparrow}_\alphanorm}
\newcommand{\cnormdown}{c^{\downarrow}_\alphanorm}
\newcommand{\cnormplus}{c^{+}_\alphanorm}

\newcommand{\diff}[1]{\textcolor{magenta}{#1}}
\newcommand{\alphain}{\alpha^{\mathrm{in}}}
\newcommand{\alphaout}{\alpha^{\mathrm{out}}}
\newcommand{\Bin}{\mathrm{Bin}}


\newcommand{\taubetadown}{\tau^\downarrow_\beta}
\newcommand{\cbetadown}{c^\downarrow_\beta}
\newcommand{\taubetaup}{\tau^\uparrow_\beta}
\newcommand{\cbetaup}{c^\uparrow_\beta}
\newcommand{\taudeltaup}{\tau^{\uparrow}_\delta}
\newcommand{\cdeltaup}{c^{\uparrow}_\delta}
\newcommand{\taudeltadown}{\tau^{\downarrow}_\delta}
\newcommand{\cdeltadown}{c^{\downarrow}_\delta}

\newcommand{\tauiup}{\tau^{\uparrow}_i}
\newcommand{\ciup}{c_\alpha^{\uparrow}}
\newcommand{\tauidown}{\tau^{\downarrow}_i}
\newcommand{\cidown}{c_\alpha^{\downarrow}}
\newcommand{\tauiweak}{\tau^{\mathrm{weak}}_i}
\newcommand{\taujweak}{\tau^{\mathrm{weak}}_j}
\newcommand{\tauijweak}{\tau^{\mathrm{weak}}_{ij}}
\newcommand{\cactive}{c^{\mathrm{active}}}

\newcommand{\taujup}{\tau^{\uparrow}_j}
\newcommand{\taujdown}{\tau^{\downarrow}_j}

\newcommand{\tauijup}{\tau^{\uparrow}_{ij}}
\newcommand{\tauijdown}{\tau^{\downarrow}_{ij}}

\newcommand{\drift}{R}
\newcommand{\tinyexists}{{}^{\exists}}
\newcommand{\tinyforall}{{}^{\forall}}
\newcommand{\alphalarge}{\zeta}
\newcommand{\taux}{\tau_X}
\newcommand{\tauxplus}{\tau_X^+}
\newcommand{\tauxminus}{\tau_X^-}
%\newcommand{\tauxup}{\tau^\uparrow_X}
%\newcommand{\tauxdown}{\tau^\downarrow_X}

\newcommand{\deltaratio}{\eta}
\newcommand{\tauetaup}{\tau^{\uparrow}_\eta}
\newcommand{\cetaup}{c^\uparrow_\eta}
\newcommand{\tauivanish}{\tau^{\mathrm{vanish}}_i}

\newcommand{\xdelta}{x_{\delta}}
\newcommand{\xeta}{x_{\eta}}

\newcommand{\vardelta}{s_{\delta}}
\newcommand{\czetaup}{c_{\zeta}^\mathrm{U}}
\newcommand{\Cdeltavarplus}{C_{\delta}}
\newcommand{\Cnorminitial}{C_{\alphanorm}}

\newcommand{\tauiactive}{\tau^{\mathrm{active}}_i}
\newcommand{\taustar}{\tau^*}

\newcommand{\xnorm}{x_{\alphanorm}}
\newcommand{\driftnorm}{\drift_{\alphanorm}}
\newcommand{\Cxdelta}{C_{x}}

\newcommand{\Csyncinitial}{C_{\mathrm{s}}}

\newcommand{\tauphiplus}{\tau_\varphi^+}
\newcommand{\tauphiup}{\tau^\uparrow_\varphi}
\newcommand{\xphiplus}{x_\varphi^+}
\newcommand{\cphiup}{c_\varphi^{\uparrow}}
\newcommand{\xphistar}{x_\varphi^*}
\newcommand{\tauphistar}{\tau_\varphi^*}

\newcommand{\hmaj}{\(h\)-majority\xspace} %h-majority dynamics
\newcommand{\threemaj}{\(3\)-Majority\xspace} %3-Majority dynamics
\newcommand{\twochoices}{\(2\)-Choices\xspace} %2-Choices dynamics
\newcommand{\undecided}{Undecided-State\xspace}
\newcommand{\conf}{\mathbf{c}} % configuration of the system
\newcommand{\bias}{\mathrm{B}} % bias of the system

